Estimation of geodesic tortuosity and constrictivity in stationary random closed sets

We investigate the problem of estimating geodesic tortuosity and constrictivity as two structural characteristics of stationary random closed sets. They are of central importance for the analysis of effective transport properties in porous or composite materials. Loosely speaking, geodesic tortuosity measures the windedness of paths whereas the notion of constrictivity captures the appearance of bottlenecks resulting from narrow passages within a given materials phase. We first provide mathematically precise definitions of these quantities and introduce appropriate estimators. Then, we show strong consistency of these estimators for unboundedly growing sampling windows. In order to apply our estimators to real datasets, the extent of edge effects needs to be controlled. This is illustrated using a model for a multi-phase material that is incorporated in solid oxid fuel cells.

==> estimation.tex <==
In this section, we consider discrete image data on a $3$D grid $\mathbb{Z}_h^3\cap W$, where $W$ denotes an observation window, $\mathbb{Z}_h^3=\{hz: z\in\mathbb{Z}^3\}$ and $h>0$ (resolution of the image). For simplification consider such $h$ that there exists $n\in\mathbb{N}$ satisfies $nh=l$.


\subsection{Mean geodesic tortuosity}
For estimation of mean geodesic tortuosity we consider a discretization of image data, such that $v$ coincides with $e_3$. For estimating $\tau_{v,l}$ on the basis of a 3D image or of discretized realizations of random sets we approximate the path lengths in transport direction on the voxel grid. 
For this purpose we consider all voxels in $\Xi$ as vertices of a graph $G=(V,E)$ with vertex set $V = \mathbb{Z}_h^{3} \cap \Xi \cap W^l$ and edge set $E$, where $W^l=[0,w_1]\times[0,w_2]\times[0,l]$. In this graph each vertex is connected by an edge to all other vertices in its 26-neighborhood, i.e. $E= \lbrace (x,y) : x,y \in V, 0 <|x-y| \leq h \sqrt{3} \rbrace$. We estimate $\tau_{v,l}$ by computing the shortest path length on the graph $G$ by Dijkstra's algorithm, see e.g. \cite{thulasiraman.1992}. A shortest path through $\Xi$ on a grid is visualized in Figure \ref{fig:tortuosity}.

\begin{figure}[h]
	\begin{center}
	\includegraphics[width=4cm]{figures/tortuosity/Folie6_crop.png}
	\includegraphics[width=4cm]{figures/tortuosity/Folie5_crop.png}
	\caption{Left: 2D-visualization of the shortest path in $\Xi$, represented in gray, from the $W_{I}$ to $W_{O}$. Right: Approximation of the shortest path on a grid. Both transport paths are represented in orange. Note that 2D structures are shown for a better visualization, while all computations are done in 3D.}\label{fig:tortuosity}
	\end{center}
\end{figure}

For a formal definition of the estimator, we write $x \sim y$ for vertices $x,y \in V$ if there is a path from $x$ to $y$ in $G$, i.e. if there exists an integer $n \geq 2$ and a sequence $x=x_{1}, \ldots, x_{n}=y$ such that $(x_{j}, x_{j+1}) \in E$ for each $j \in \lbrace 1, \ldots, n-1 \rbrace$. Denote $W_I=\{(x_1,x_2,x_3)\in W^l:x_3=0\}$, $W_O=\{(x_1,x_2,x_3)\in W^l:x_3=l\}$ and $W'_{I, \Xi}=\lbrace x \in \mathbb{Z}_h^{3} \cap \Xi \cap W_{I}: \text{It exists } y \in W_{O}, x \sim y \rbrace$ the set of vertices in $W_{I}$ for which there is a path to $W_{O}$ in $G$.

 With this notation the formal definition of the estimator $\widehat{\tau}_{v,l}$ is given by
$$ \widehat{\tau}_{v,l} = \frac{1}{\#W'_{I,\Xi}} \sum_{x \in W'_{I,\Xi}} \min_{y \in W_{O}} \min_{\substack{ n\geq 2, \, x = x_{1}, \ldots, x_{n} = y  \\ (x_{1},x_{2}), \ldots, (x_{n-1}, x_{n}) \in E }} \sum_{j=1}^{n-1} | x_{j} - x_{j+1} |,$$ where we use the convention $\min_{x \in \emptyset} g(x) = \infty$ for any function $g$ and $\# A$ denotes the cardinality of the set $A$.  


\subsection{Constrictivity}
Note that the definition of $r_{\max}$ does not depend on the observation window $W$ since $\Xi$ was assumed to be stationary. Using morphological opening on experimental image data and discretized realizations of random sets  the estimation of $r_{\max}$ reduces to the estimation of volume fractions $p$, where $p(\Xi)=\mathbb{E}\nu_{3}(\Xi\cap [0,1]^3)$. 
The estimation of volume fraction is given by $\widehat{p} = \sum_{x \in \mathbb{Z}^{3} \cap W} \mathbb{I}(x \in \Xi) / \# (\mathbb{Z}^{3} \cap W),$ where $\mathbb{I}$ denotes the indicator function .

For the estimation of $r_{\min, W}$ we have also determine the subset of $(\Xi \ominus \bar{B}(o,r)) \cap W$ which is connected to $W_{I}$. A description for the algorithmic estimation of $r_ {\min, W}$ can be found in \cite{muench.2008}. 










==> sketch_proof_monotonicity_granulometry.tex <==
\begin{figure}
\begin{tikzpicture}


\newcommand*\kante{0.75}
% Ecken
\path[scale=\kante]
  (1.00,1.06,0.90) coordinate (C1)
  (1.08,1.10,-1.12) coordinate (G1)
  (0.85,-1.12,0.91) coordinate (B1)
  (-1.11,0.90,0.94) coordinate (D1)
  (0.96,-1.01,-1.00) coordinate (F1)
  (-1.08,1.10,-0.90) coordinate (H1)
  (-1.08,-0.86,0.91) coordinate (A1)
  (-0.87,-0.98,-0.90) coordinate (E1)
  
  (1.65,1.59,1.53) coordinate (C2)
  (1.43,1.56,-1.55) coordinate (G2)
  (1.64,-1.36,1.59) coordinate (B2)
  (-1.55,1.38,1.36) coordinate (D2)
  (1.51,-1.57,-1.38) coordinate (F2)
  (-1.39,1.64,-1.41) coordinate (H2)
  (-1.59,-1.50,1.42) coordinate (A2)
  (-1.53,-1.50,-1.42) coordinate (E2)
  


  (2.87,3.04,3.01) coordinate (C3)
  (3.10,3.08,-3.00) coordinate (G3)
  (2.97,-3.01,2.95) coordinate (B3)
  (-3.11,2.94,2.94) coordinate (D3)
  (3.10,-2.94,-3.09) coordinate (F3)
  (-2.92,2.87,-3.00) coordinate (H3)
  (-3.07,-2.96,3.08) coordinate (A3)
  (-2.87,-2.89,-3.15) coordinate (E3)
  
;
%Kanten
\draw[font=\tiny]
  (A1) -- node[above]{}  (B1) -- node[above]{} (C1)
      -- (D1) -- cycle
  (B1) -- node[above]{}(F1)
      -- (G1) -- (H1) --(D1)
  (C1) -- (G1)
;
\path[very thin] (E1) edge (A1) edge (F1) edge (H1);

\draw[font=\tiny,  blue]
(A2) -- node[above]{}  (B2) -- node[above]{} (C2)
-- (D2) -- cycle
(B2) -- node[above]{}(F2)
-- (G2) -- (H2) --(D2)
(C2) -- (G2)
;
\path[very thin, blue] (E2) edge (A2) edge (F2) edge (H2);

\draw[font=\tiny,  blue]
(A3) -- node[above]{}  (B3) -- node[above]{} (C3)
-- (D3) -- cycle
(B3) -- node[above]{}(F3)
-- (G3) -- (H3) --(D3)
(C3) -- (G3)
;
\path[ very thin, blue] (E3) edge (A3) edge (F3) edge (H3);

\path[font=\tiny,  blue] (A2) edge (A3);
\path[font=\tiny,  blue] (B2) edge (B3);
\path[font=\tiny,  blue] (C2) edge (C3);
\path[font=\tiny,  blue] (D2) edge (D3);
\path[font=\tiny,  blue] (E2) edge (E3);
\path[font=\tiny,  blue] (F2) edge (F3);
\path[font=\tiny,  blue] (G2) edge (G3);
\path[font=\tiny,  blue] (H2) edge (H3);
\end{tikzpicture}
\caption{Visualization of a realization contained in $A$ with $k = 2$. The edges of $\Rng(\vy_{1}, \ldots, \vy_{8})$ are drawn in black, while the edges of $\Rng(\widetilde{\vy}_{1}, \ldots, \widetilde{\vy}_{16})$ are drawn in blue.}\label{fig:sketch_proof_app2}
\end{figure}
